Dwarfs in nearby voids: results of SALT spectroscopy

In the framework of the ongoing project, aimed at the systematical studying galaxies in nearby voids, we conducted spectroscopy with the Southern African Large Telescope (SALT) of 62 objects from the Nearby Void Galaxy (NVG) sample. They include 8 remaining objects of the 60 preselected candidates to eXtremely Metal-Poor (XMP) dwarfs, two known void XMP dwarfs and 52 void dwarfs residing within the Local Volume. For 47 galaxies residing in the nearby voids, we obtained spectra of the diverse quality. For 42 of them, we detected the Hydrogen and Oxygen lines that allowed us to get estimates of O/H in the observed HII regions. For 12 of the 42 objects, we detected the faint line [Oiii]4363, that allowed us to directly derive the electron temperature T_e and obtain their gas O/H by the direct method. 14 objects with the undetected [Oiii]4363 line fall to the lowest metallicities range (12+log(O/H) < 7.5 dex). For them, we use a carefully checked new empirical 'Strong line' method of Izotov et al. For 14 other objects with only strong lines detected and with 12+log(O/H) of ~7.5-8.0 dex, we used the modified version of 'semi-empirical' method of Izotov and Thuan. It accounts for effect of the excitation parameter O32 on T_e. 16 new galaxies are found with parameter 12+log(O/H) < 7.39 dex. Of them, four have 12+log(O/H) = 7.07 - 7.20 dex. Of the 60 observed NVG objects, 15 have mistaken radial velocities in HyperLEDA. They do not reside in the nearby voids.

==> addtab.tex <==
%J0015+0104_dir.tex
%J0026_ESO294-010.tex
%J0108_PGC004055a.tex
\begin{table*}
\centering{
\caption{Line intensities and derived parameters of J0015+0104, ESO294-010 and PGC004055}
\label{t:Intens1}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{J0015+0104=J0015+0104 }    % \\ \hline
& \MC{2}{c}{ESO294-010=J0026--4151}    % \\ \hline
& \MC{2}{c}{PGC004055=J0108--3812}       \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                   &  1.455$\pm$ 0.053 &  1.456$\pm$ 0.058  &  2.568$\pm$ 0.240 &  2.120$\pm$ 0.267  &  1.873$\pm$ 0.050 &  1.792$\pm$ 0.058        \\
3868\ [Ne\ {\sc iii}]\                 &        ...        &        ...         &        ...        &        ...         &  0.155$\pm$ 0.007 &  0.147$\pm$ 0.008        \\ 
3889\ He\ {\sc i}\ +\ H8\              &        ...        &        ...         &        ...        &        ...         &  0.050$\pm$ 0.011 &  0.238$\pm$ 0.081        \\ 
4101\ H$\delta$\                       &  0.206$\pm$ 0.016 &  0.250$\pm$ 0.025  &        ...        &        ...         &  0.102$\pm$ 0.011 &  0.269$\pm$ 0.042        \\ 
4340\ H$\gamma$\                       &  0.449$\pm$ 0.024 &  0.484$\pm$ 0.030  &  0.221$\pm$ 0.055 &  0.335$\pm$ 0.134  &  0.354$\pm$ 0.025 &  0.469$\pm$ 0.039        \\
4363\ [O\ {\sc iii}]\                  &  0.028$\pm$ 0.017 &  0.028$\pm$ 0.017  &        ...        &        ...         &  0.025$\pm$ 0.014 &  0.023$\pm$ 0.015        \\ 
4861\ H$\beta$\                        &  1.000$\pm$ 0.041 &  1.000$\pm$ 0.043  &  1.000$\pm$ 0.122 &  1.000$\pm$ 0.193  &  1.000$\pm$ 0.029 &  1.000$\pm$ 0.034        \\
4959\ [O\ {\sc iii}]\                  &  0.239$\pm$ 0.017 &  0.231$\pm$ 0.017  &  1.221$\pm$ 0.136 &  1.008$\pm$ 0.138  &  0.624$\pm$ 0.020 &  0.551$\pm$ 0.020        \\
5007\ [O\ {\sc iii}]\                  &  0.716$\pm$ 0.027 &  0.692$\pm$ 0.027  &  3.316$\pm$ 0.302 &  2.737$\pm$ 0.256  &  2.068$\pm$ 0.056 &  1.821$\pm$ 0.055        \\
6548\ [N\ {\sc ii}]\                   &  0.014$\pm$ 0.004 &  0.013$\pm$ 0.004  &  0.095$\pm$ 0.179 &  0.078$\pm$ 0.179  &  0.030$\pm$ 0.017 &  0.025$\pm$ 0.016        \\
6563\ H$\alpha$\                       &  2.878$\pm$ 0.094 &  2.712$\pm$ 0.099  &  3.210$\pm$ 0.362 &  2.799$\pm$ 0.421  &  3.381$\pm$ 0.090 &  2.830$\pm$ 0.092        \\
6584\ [N\ {\sc ii}]\                   &  0.043$\pm$ 0.012 &  0.040$\pm$ 0.011  &  0.316$\pm$ 0.212 &  0.261$\pm$ 0.212  &  0.100$\pm$ 0.023 &  0.082$\pm$ 0.021        \\
%                                                                                                                        
   &  &  &  &  & & \\                                                                                                    
C(H$\beta$)\ dex                       & \MC {2}{c}{0.04$\pm$0.04}              & \MC {2}{c}{0.00$\pm$0.15}              & \MC {2}{c}{0.10$\pm$0.03}                    \\
EW(abs)\ \AA\                          & \MC {2}{c}{1.45$\pm$0.45}              & \MC {2}{c}{0.40$\pm$0.16}              & \MC {2}{c}{3.00$\pm$0.15}                    \\
EW(H$\beta$)\ \AA\                     & \MC {2}{c}{ 46.2$\pm$1.3}              & \MC {2}{c}{  1.9$\pm$0.14}             & \MC {2}{c}{23.8$\pm$0.5}                      \\
\hline                                                                                                                                     
$T_{\rm e}$(OIII)(K)\                  & \MC {2}{c}{22364$\pm$9155}             & \MC {2}{c}{14354$\pm$1209}             & \MC {2}{c}{12753$\pm$3097}                   \\
$T_{\rm e}$(OII)(K)\                   & \MC {2}{c}{16280$\pm$1897}             & \MC {2}{c}{13551$\pm$709 }             & \MC {2}{c}{12456$\pm$2422}                   \\
O$^{+}$/H$^{+}$($\times$10$^5$)\       & \MC {2}{c}{1.033$\pm$0.351}            & \MC {2}{c}{2.665$\pm$0.576}            & \MC {2}{c}{3.020$\pm$2.114}                  \\
O$^{++}$/H$^{+}$($\times$10$^5$)\      & \MC {2}{c}{0.317$\pm$0.248}            & \MC {2}{c}{3.455$\pm$0.803}            & \MC {2}{c}{3.021$\pm$2.092}                  \\
O/H($\times$10$^5$)\                   & \MC {2}{c}{1.350$\pm$0.430}            & \MC {2}{c}{6.120$\pm$0.987}            & \MC {2}{c}{6.041$\pm$2.974}                  \\
12+log(O/H)(d)\                        & \MC {2}{c}{7.13$\pm$0.14}              & \MC {2}{c}{...          }              & \MC {2}{c}{7.78$\pm$0.21}                    \\
12+log(O/H)(s)\                        & \MC {2}{c}{7.14$\pm$0.05}              & \MC {2}{c}{...          }              & \MC {2}{c}{...          }                    \\
12+log(O/H)(mse,c)\                    & \MC {2}{c}{7.18$\pm$0.11}              & \MC {2}{c}{7.79$\pm$0.12}              & \MC {2}{c}{7.53$\pm$0.11}                    \\
12+log(O/H)(PT05)\                     & \MC {2}{c}{...          }              & \MC {2}{c}{7.84$\pm$0.10}              & \MC {2}{c}{7.63$\pm$0.10}                    \\
\MC{3}{l}{~~} \
\end{tabular}
 }
\end{table*}

%J0231_AGC124137c.tex
%J0258_ESO199-007a.tex
%J0306_PGC1166738
\begin{table*}
\centering{
\caption{Line intensities and derived parameters of UGC01085, AGC124137 and ESO199-007}
\label{t:Intens2}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{UGC01085=J0131+0747}      % \\ \hline
& \MC{2}{c}{AGC124137=J0231+0931  }   % \\ \hline
& \MC{2}{c}{ESO199-007=J0258--4922}    \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  2.434$\pm$ 0.097 &  2.272$\pm$ 0.110  &  2.440$\pm$ 0.521 &  1.289$\pm$ 0.688  &  1.169$\pm$ 0.040 &  1.089$\pm$ 0.044  \\
3868\ [Ne\ {\sc iii}]\              &        ...        &        ...         &        ...        &        ...         &  0.156$\pm$ 0.014 &  0.145$\pm$ 0.014  \\ 
3889\ He\ {\sc i}\ +\ H8\           &        ...        &        ...         &        ...        &        ...         &  0.143$\pm$ 0.013 &  0.253$\pm$ 0.033  \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\       &        ...        &        ...         &        ...        &        ...         &  0.130$\pm$ 0.013 &  0.246$\pm$ 0.036  \\ 
4101\ H$\delta$\                    &  0.133$\pm$ 0.022 &  0.277$\pm$ 0.063  &        ...        &        ...         &  0.143$\pm$ 0.013 &  0.240$\pm$ 0.030  \\
4340\ H$\gamma$\                    &  0.355$\pm$ 0.098 &  0.449$\pm$ 0.149  &  0.028$\pm$ 0.165 &  0.479$\pm$ 9.148  &  0.403$\pm$ 0.040 &  0.483$\pm$ 0.056  \\
4471\ He\ {\sc i}\                  &        ...        &        ...         &        ...        &        ...         &  0.065$\pm$ 0.013 &  0.059$\pm$ 0.013  \\ 
4861\ H$\beta$\                     &  1.000$\pm$ 0.040 &  1.000$\pm$ 0.091  &  1.000$\pm$ 0.259 &  1.000$\pm$ 2.721  &  1.000$\pm$ 0.037 &  1.000$\pm$ 0.042  \\
4959\ [O\ {\sc iii}]\               &  1.248$\pm$ 0.046 &  1.079$\pm$ 0.046  &  0.431$\pm$ 0.251 &  0.181$\pm$ 0.249  &  0.714$\pm$ 0.023 &  0.648$\pm$ 0.023  \\
5007\ [O\ {\sc iii}]\               &  3.613$\pm$ 0.114 &  3.117$\pm$ 0.113  &  1.303$\pm$ 0.338 &  0.543$\pm$ 0.332  &  2.234$\pm$ 0.070 &  2.026$\pm$ 0.070  \\
6548\ [N\ {\sc ii}]\                &  0.034$\pm$ 0.030 &  0.027$\pm$ 0.028  &        ...        &        ...         &  0.000$\pm$ 0.013 &  0.000$\pm$ 0.013  \\
6563\ H$\alpha$\                    &  3.399$\pm$ 0.115 &  2.808$\pm$ 0.119  &  6.670$\pm$ 1.249 &  2.716$\pm$ 2.457  &  3.052$\pm$ 0.095 &  2.763$\pm$ 0.103  \\
6584\ [N\ {\sc ii}]\                &  0.138$\pm$ 0.041 &  0.111$\pm$ 0.038  &        ...        &        ...         &  0.039$\pm$ 0.026 &  0.035$\pm$ 0.025  \\
%                                                                                                                     
   &  &  &  &  & & \\                                                                                                 
C(H$\beta$)\ dex                    & \MC {2}{c}{0.01$\pm$0.04}              & \MC {2}{c}{0.30$\pm$0.24}              & \MC {2}{c}{0.04$\pm$0.04}              \\
EW(abs)\ \AA\                       & \MC {2}{c}{2.65$\pm$0.23}              & \MC {2}{c}{1.45$\pm$2.84}              & \MC {2}{c}{4.40$\pm$0.53}              \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{17.7$\pm$0.5}               & \MC {2}{c}{ 1.1$\pm$0.2}               & \MC {2}{c}{44.1$\pm$0.9}               \\
\hline                                                                                                                
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{13889$\pm$1164}             & \MC {2}{c}{22582$\pm$3630}             & \MC {2}{c}{17503$\pm$2273}             \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{13265$\pm$749 }             & \MC {2}{c}{16324$\pm$723 }             & \MC {2}{c}{14794$\pm$461 }             \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{3.071$\pm$0.610}            & \MC {2}{c}{0.907$\pm$0.498}            & \MC {2}{c}{1.031$\pm$0.108}            \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{4.223$\pm$0.952}            & \MC {2}{c}{0.244$\pm$0.158}            & \MC {2}{c}{1.526$\pm$0.448}            \\
O/H($\times$10$^5$)\                & \MC {2}{c}{7.294$\pm$1.131}            & \MC {2}{c}{1.151$\pm$0.522}            & \MC {2}{c}{2.557$\pm$0.461}            \\
12+log(O/H)(s)\                     & \MC {2}{c}{...          }              & \MC {2}{c}{7.08$\pm$0.17}              & \MC {2}{c}{7.33$\pm$0.05}              \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.87$\pm$0.11}              & \MC {2}{c}{7.10$\pm$0.20}              & \MC {2}{c}{7.43$\pm$0.12}              \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{7.92$\pm$0.10}              & \MC {2}{c}{...          }              & \MC {2}{c}{7.49$\pm$0.10}              \\
\MC{3}{l}{~~} \                                                                                                                  
\end{tabular}                                                                                                                    
 }
\end{table*}

%J0335_PGC013294a.tex
%J0339_PGC681755c.tex
%J0410_ESO359-024.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC1166738, PGC013294 and PGC681755}
\label{t:Intens3}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC1166738=J0306+0028 }    % \\ \hline
& \MC{2}{c}{PGC013294=J0335--4511}    % \\ \hline
& \MC{2}{c}{PGC681755=J0339--3303}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  1.416$\pm$ 0.090 &  1.208$\pm$ 0.113  &  2.403$\pm$ 0.066 &  2.401$\pm$ 0.073  &  6.298$\pm$ 0.485 &  4.431$\pm$ 0.611   \\
3967\ [Ne\ {\sc iii}]\ +\ H7\       &        ...        &        ...         &  0.159$\pm$ 0.008 &  0.160$\pm$ 0.011  &        ...        &        ...          \\ 
4101\ H$\delta$\                    &  0.133$\pm$ 0.041 &  0.521$\pm$ 0.292  &  0.202$\pm$ 0.010 &  0.203$\pm$ 0.012  &        ...        &        ...          \\
4340\ H$\gamma$\                    &  0.040$\pm$ 0.023 &  0.414$\pm$ 0.443  &  0.400$\pm$ 0.015 &  0.401$\pm$ 0.016  &  0.172$\pm$ 0.047 &  0.476$\pm$ 0.255   \\
4363\ [O\ {\sc iii}]\               &        ...        &        ...         &  0.038$\pm$ 0.007 &  0.038$\pm$ 0.007  &        ...        &        ...          \\ 
4861\ H$\beta$\                     &  1.000$\pm$ 0.056 &  1.000$\pm$ 0.110  &  1.000$\pm$ 0.038 &  1.000$\pm$ 0.038  &  1.000$\pm$ 0.105 &  1.000$\pm$ 0.179   \\ 
4959\ [O\ {\sc iii}]\               &  0.445$\pm$ 0.039 &  0.313$\pm$ 0.039  &  0.917$\pm$ 0.030 &  0.916$\pm$ 0.030  &  0.545$\pm$ 0.066 &  0.342$\pm$ 0.066   \\
5007\ [O\ {\sc iii}]\               &  1.387$\pm$ 0.073 &  0.969$\pm$ 0.072  &  2.673$\pm$ 0.076 &  2.671$\pm$ 0.076  &  1.776$\pm$ 0.152 &  1.111$\pm$ 0.151   \\
%6548\ [N\ {\sc ii}]\                &  0.019$\pm$ 0.090 &  0.009$\pm$ 0.080  &  0.004$\pm$ 0.004 &  0.004$\pm$ 0.004  &        ...        &        ...          \\
%6548\ [N\ {\sc ii}]\                &  0.019$\pm$ 0.090 &  0.009$\pm$ 0.080  &  0.042$\pm$ 0.007 &  0.042$\pm$ 0.007  &  0.119$\pm$ 0.172 &  0.067$\pm$ 0.154   \\
6563\ H$\alpha$\                    &  4.405$\pm$ 0.209 &  2.735$\pm$ 0.199  &  2.823$\pm$ 0.091 &  2.821$\pm$ 0.099  &  4.440$\pm$ 0.441 &  2.771$\pm$ 0.475   \\
%6584\ [N\ {\sc ii}]\                &  0.060$\pm$ 0.098 &  0.030$\pm$ 0.086  &  0.138$\pm$ 0.015 &  0.138$\pm$ 0.015  &  0.403$\pm$ 0.233 &  0.227$\pm$ 0.209   \\
%                                                                                                                     
   &  &  &  &  & & \\                                                                                                 
C(H$\beta$)\ dex                    & \MC {2}{c}{0.26$\pm$0.06}              & \MC {2}{c}{0.00$\pm$0.04}              & \MC {2}{c}{0.15$\pm$0.13}               \\
EW(abs)\ \AA\                       & \MC {2}{c}{1.60$\pm$0.02}              & \MC {2}{c}{0.05$\pm$0.28}              & \MC {2}{c}{1.15$\pm$0.09}               \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{4.0$\pm$ 0.2}               & \MC {2}{c}{59.1$\pm$1.6}               & \MC {2}{c}{ 2.0$\pm$0.2}                \\
\hline                                                                                                                                                              
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{20295$\pm$2294}             & \MC {2}{c}{13134$\pm$988 }             & \MC {2}{c}{17522$\pm$2283}              \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{15627$\pm$100 }             & \MC {2}{c}{12745$\pm$727 }             & \MC {2}{c}{14798$\pm$457 }              \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{0.967$\pm$0.092}            & \MC {2}{c}{3.728$\pm$0.759}            & \MC {2}{c}{4.190$\pm$0.705}             \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{0.533$\pm$0.127}            & \MC {2}{c}{4.204$\pm$0.886}            & \MC {2}{c}{0.827$\pm$0.260}             \\
O/H($\times$10$^5$)\                & \MC {2}{c}{1.500$\pm$0.157}            & \MC {2}{c}{7.933$\pm$1.166}            & \MC {2}{c}{5.017$\pm$0.752}             \\
12+log(O/H)(d)\                     & \MC {2}{c}{... }                       & \MC {2}{c}{7.90$\pm$0.06}              & \MC {2}{c}{... }                        \\
12+log(O/H)(s)\                     & \MC {2}{c}{7.16$\pm$0.05}              & \MC {2}{c}{...}                        & \MC {2}{c}{...}                         \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.21$\pm$0.13}              & \MC {2}{c}{7.83$\pm$0.11}              & \MC {2}{c}{7.71$\pm$0.11:}              \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{...          }              & \MC {2}{c}{7.88$\pm$0.10}              & \MC {2}{c}{... }                        \\
\MC{3}{l}{~~} \
\end{tabular}
 }
\end{table*}

%J0456_PGC016389b.tex
%J0517_HIPASSJ0517b.tex
%J0527_ESO553-046c.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of ESO359-024, PGC016389 and HIPASSJ0517-32}
\label{t:Intens4}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{ESO359-024=J0410--3549    }    % \\ \hline
& \MC{2}{c}{PGC016389a=J0456--4248     }    % \\ \hline
& \MC{2}{c}{HIPASSJ0517-32=J0517--3245}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  3.631$\pm$ 0.117 &  3.342$\pm$ 0.143  &  1.566$\pm$ 0.073 &  1.273$\pm$ 0.143  &  2.449$\pm$ 0.050 &  2.711$\pm$ 0.064  \\
3868\ [Ne\ {\sc iii}]\              &  0.134$\pm$ 0.029 &  0.121$\pm$ 0.032  &        ...        &        ...         &  0.371$\pm$ 0.018 &  0.401$\pm$ 0.021  \\ 
3889\ He\ {\sc i}\ +\ H8\           &        ...        &        ...         &        ...        &        ...         &  0.040$\pm$ 0.011 &  0.143$\pm$ 0.053  \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\       &        ...        &        ...         &        ...        &        ...         &  0.082$\pm$ 0.006 &  0.178$\pm$ 0.016  \\ 
4101\ H$\delta$\                    &        ...        &        ...         &  0.026$\pm$ 0.022 &  0.287$\pm$ 0.409  &  0.159$\pm$ 0.007 &  0.257$\pm$ 0.014  \\
4340\ H$\gamma$\                    &  0.307$\pm$ 0.057 &  0.479$\pm$ 0.130  &  0.243$\pm$ 0.024 &  0.415$\pm$ 0.074  &  0.391$\pm$ 0.016 &  0.471$\pm$ 0.021  \\
4363\ [O\ {\sc iii}]\               &  0.079$\pm$ 0.048 &  0.068$\pm$ 0.051  &        ...        &        ...         &  0.054$\pm$ 0.012 &  0.054$\pm$ 0.013  \\ 
4861\ H$\beta$\                     &  1.000$\pm$ 0.035 &  1.000$\pm$ 0.063  &  1.000$\pm$ 0.052 &  1.000$\pm$ 0.076  &  1.000$\pm$ 0.019 &  1.000$\pm$ 0.022  \\
4959\ [O\ {\sc iii}]\               &  0.562$\pm$ 0.024 &  0.457$\pm$ 0.024  &  0.125$\pm$ 0.026 &  0.102$\pm$ 0.026  &  1.186$\pm$ 0.022 &  1.089$\pm$ 0.022  \\
5007\ [O\ {\sc iii}]\               &  1.841$\pm$ 0.062 &  1.488$\pm$ 0.062  &  0.302$\pm$ 0.031 &  0.245$\pm$ 0.031  &  3.574$\pm$ 0.066 &  3.264$\pm$ 0.065  \\
6300\ [O\ {\sc i}]\                 &  0.038$\pm$ 0.039 &  0.028$\pm$ 0.035  &        ...        &        ...         &  0.062$\pm$ 0.011 &  0.049$\pm$ 0.009  \\ 
6312\ [S\ {\sc iii}]\               &  0.006$\pm$ 0.029 &  0.005$\pm$ 0.026  &        ...        &        ...         &  0.039$\pm$ 0.012 &  0.030$\pm$ 0.010  \\ 
6548\ [N\ {\sc ii}]\                &  0.060$\pm$ 0.047 &  0.043$\pm$ 0.041  &        ...        &        ...         &  0.034$\pm$ 0.010 &  0.026$\pm$ 0.008  \\
6563\ H$\alpha$\                    &  3.584$\pm$ 0.120 &  2.693$\pm$ 0.123  &  3.287$\pm$ 0.129 &  2.757$\pm$ 0.145  &  3.591$\pm$ 0.066 &  2.812$\pm$ 0.060  \\
6584\ [N\ {\sc ii}]\                &  0.184$\pm$ 0.053 &  0.133$\pm$ 0.047  &        ...        &        ...         &  0.105$\pm$ 0.013 &  0.081$\pm$ 0.011  \\
%                                                                                                                     
   &  &  &  &  & & \\                                                                                                 
C(H$\beta$)\ dex                    & \MC {2}{c}{0.17$\pm$0.04}               & \MC {2}{c}{0.00$\pm$0.05}               & \MC {2}{c}{0.24$\pm$0.02}             \\
EW(abs)\ \AA\                       & \MC {2}{c}{2.25$\pm$0.46}               & \MC {2}{c}{1.40$\pm$0.25}               & \MC {2}{c}{1.65$\pm$0.11}             \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{10.2$\pm$0.3}                & \MC {2}{c}{ 6.1$\pm$0.2}                & \MC {2}{c}{22.2$\pm$0.3}              \\
\hline                                                                                                                                                          
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{24796$\pm$13957}             & \MC {2}{c}{18314$\pm$1356}              & \MC {2}{c}{14038$\pm$1427}            \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{16675$\pm$1641}              & \MC {2}{c}{15345$\pm$327 }              & \MC {2}{c}{13360$\pm$893 }            \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{2.213$\pm$0.627}             & \MC {2}{c}{1.076$\pm$0.095}             & \MC {2}{c}{3.576$\pm$0.815}           \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{0.552$\pm$0.557}             & \MC {2}{c}{0.179$\pm$0.036}             & \MC {2}{c}{4.259$\pm$1.148}           \\
O/H($\times$10$^5$)\                & \MC {2}{c}{2.765$\pm$0.838}             & \MC {2}{c}{1.255$\pm$0.102}             & \MC {2}{c}{7.836$\pm$1.408}           \\
12+log(O/H)(d)\                     & \MC {2}{c}{7.44$\pm$0.13}               & \MC {2}{c}{... }                        & \MC {2}{c}{7.89$\pm$0.08}             \\
12+log(O/H)(s)\                     & \MC {2}{c}{7.48$\pm$0.04}               & \MC {2}{c}{6.98$\pm$0.05}               & \MC {2}{c}{...          }             \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.66$\pm$0.12}               & \MC {2}{c}{7.13$\pm$0.10}               & \MC {2}{c}{7.96$\pm$0.12}             \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{... }                        & \MC {2}{c}{... }                        & \MC {2}{c}{8.03$\pm$0.10}             \\
\MC{3}{l}{~~} \
\end{tabular}
 }
\end{table*}


%J0557_PGC138836a.tex
%J0607_PGC018431a.tex
%J0639_ESO308-022c.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of ESO553-046, PGC138836 and PGC018431}
\label{t:Intens5}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{ESO553-046=J0527--2040}    % \\ \hline
& \MC{2}{c}{PGC138836=J0557+0729  }    % \\ \hline
& \MC{2}{c}{PGC018431=J0607--3412 }      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  1.990$\pm$ 0.039 &  2.027$\pm$ 0.044  &  1.049$\pm$ 0.077 &  1.537$\pm$ 0.144  &  3.350$\pm$ 0.097 &  3.205$\pm$ 0.104  \\ 
3750\ H12\                          &  0.017$\pm$ 0.002 &  0.064$\pm$ 0.009  &        ...        &        ...         &        ...        &        ...         \\  
3770\ H11\                          &  0.021$\pm$ 0.001 &  0.067$\pm$ 0.005  &        ...        &        ...         &        ...        &        ...         \\  
3798\ H10\                          &  0.022$\pm$ 0.002 &  0.069$\pm$ 0.006  &        ...        &        ...         &        ...        &        ...         \\  
3835\ H9\                           &  0.046$\pm$ 0.002 &  0.093$\pm$ 0.005  &        ...        &        ...         &        ...        &        ...         \\  
3868\ [Ne\ {\sc iii}]\              &  0.356$\pm$ 0.009 &  0.360$\pm$ 0.009  &        ...        &        ...         &  0.192$\pm$ 0.007 &  0.184$\pm$ 0.007  \\  
3889\ He\ {\sc i}\ +\ H8\           &  0.162$\pm$ 0.004 &  0.210$\pm$ 0.006  &        ...        &        ...         &  0.068$\pm$ 0.011 &  0.121$\pm$ 0.022  \\  
3967\ [Ne\ {\sc iii}]\ +\ H7\       &  0.217$\pm$ 0.005 &  0.263$\pm$ 0.007  &        ...        &        ...         &        ...        &        ...         \\  
4026\ He\ {\sc i}\                  &  0.008$\pm$ 0.001 &  0.008$\pm$ 0.001  &        ...        &        ...         &        ...        &        ...         \\ 
4068\ [S\ {\sc ii}]\                &  0.017$\pm$ 0.001 &  0.017$\pm$ 0.001  &        ...        &        ...         &        ...        &        ...         \\  
4101\ H$\delta$\                    &  0.219$\pm$ 0.006 &  0.261$\pm$ 0.008  &  0.081$\pm$ 0.031 &  0.281$\pm$ 0.151  &  0.109$\pm$ 0.006 &  0.153$\pm$ 0.011  \\
4340\ H$\gamma$\                    &  0.439$\pm$ 0.010 &  0.469$\pm$ 0.011  &  0.263$\pm$ 0.039 &  0.460$\pm$ 0.086  &  0.342$\pm$ 0.018 &  0.368$\pm$ 0.021  \\
4363\ [O\ {\sc iii}]\               &  0.057$\pm$ 0.002 &  0.056$\pm$ 0.002  &        ...        &        ...         &  0.055$\pm$ 0.013 &  0.053$\pm$ 0.013  \\  
4471\ He\ {\sc i}\                  &  0.030$\pm$ 0.001 &  0.029$\pm$ 0.001  &        ...        &        ...         &        ...        &        ...         \\  
4861\ H$\beta$\                     &  1.000$\pm$ 0.022 &  1.000$\pm$ 0.023  &  1.000$\pm$ 0.060 &  1.000$\pm$ 0.086  &  1.000$\pm$ 0.036 &  1.000$\pm$ 0.038  \\  
4922\ He\ {\sc i}\                  &  0.010$\pm$ 0.001 &  0.009$\pm$ 0.001  &  0.863$\pm$ 0.039 &  0.730$\pm$ 0.044  &  0.780$\pm$ 0.024 &  0.747$\pm$ 0.024  \\
4959\ [O\ {\sc iii}]\               &  1.482$\pm$ 0.033 &  1.437$\pm$ 0.033  &  2.469$\pm$ 0.102 &  2.050$\pm$ 0.098  &  2.227$\pm$ 0.067 &  2.130$\pm$ 0.067  \\
5007\ [O\ {\sc iii}]\               &  4.446$\pm$ 0.096 &  4.303$\pm$ 0.095  &        ...        &        ...         &        ...        &        ...         \\  
6300\ [O\ {\sc i}]\                 &  0.040$\pm$ 0.004 &  0.037$\pm$ 0.004  &        ...        &        ...         &        ...        &        ...         \\ 
6312\ [S\ {\sc iii}]\               &  0.023$\pm$ 0.004 &  0.022$\pm$ 0.004  &        ...        &        ...         &        ...        &        ...         \\  
6364\ [O\ {\sc i}]\                 &  0.012$\pm$ 0.001 &  0.011$\pm$ 0.001  &        ...        &        ...         &        ...        &        ...         \\  
6548\ [N\ {\sc ii}]\                &  0.046$\pm$ 0.004 &  0.043$\pm$ 0.004  &  0.050$\pm$ 0.081 &  0.025$\pm$ 0.047  &  0.052$\pm$ 0.013 &  0.050$\pm$ 0.013  \\
6563\ H$\alpha$\                    &  3.041$\pm$ 0.061 &  2.828$\pm$ 0.063  &  5.388$\pm$ 0.255 &  2.793$\pm$ 0.166  &  2.872$\pm$ 0.083 &  2.771$\pm$ 0.091  \\
6584\ [N\ {\sc ii}]\                &  0.140$\pm$ 0.007 &  0.129$\pm$ 0.007  &  0.175$\pm$ 0.100 &  0.087$\pm$ 0.058  &  0.161$\pm$ 0.017 &  0.154$\pm$ 0.017  \\
6678\ He\ {\sc i}\                  &  0.028$\pm$ 0.001 &  0.026$\pm$ 0.001  &        ...        &        ...         &        ...        &        ...         \\  
%                                                                                                                     
   &  &  &  &  & & \\                                                                                                 
C(H$\beta$)\ dex                    & \MC {2}{c}{0.07$\pm$0.03}              & \MC {2}{c}{0.74$\pm$0.06}               & \MC {2}{c}{0.00$\pm$0.04}             \\
EW(abs)\ \AA\                       & \MC {2}{c}{2.60$\pm$0.09}              & \MC {2}{c}{4.75$\pm$0.47}               & \MC {2}{c}{0.90$\pm$0.08}             \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{93.1$\pm$1.5}               & \MC {2}{c}{34.6$\pm$1.4}                & \MC {2}{c}{19.8$\pm$0.5}              \\
\hline                                                                                                                                                             
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{12756$\pm$182 }             & \MC {2}{c}{16143$\pm$1208}              & \MC {2}{c}{16770$\pm$2153}            \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{12458$\pm$142 }             & \MC {2}{c}{14406$\pm$445 }              & \MC {2}{c}{14613$\pm$629 }            \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{3.413$\pm$0.159}            & \MC {2}{c}{1.619$\pm$0.274}             & \MC {2}{c}{3.152$\pm$0.440}           \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{7.305$\pm$0.323}            & \MC {2}{c}{1.914$\pm$0.350}             & \MC {2}{c}{1.811$\pm$0.542}           \\
O/H($\times$10$^5$)\                & \MC {2}{c}{10.720$\pm$0.360}           & \MC {2}{c}{3.533$\pm$0.444}             & \MC {2}{c}{4.964$\pm$0.698}           \\
12+log(O/H)(d)\                     & \MC {2}{c}{8.03$\pm$0.01}              & \MC {2}{c}{...}                         & \MC {2}{c}{7.70$\pm$0.06}             \\
%12+log(O/H)(s)\                     & \MC {2}{c}{...}                        & \MC {2}{c}{...}                         & \MC {2}{c}{...}                       \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{8.03$\pm$0.09}              & \MC {2}{c}{7.56$\pm$0.10}               & \MC {2}{c}{7.97$\pm$0.12}             \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{8.01$\pm$0.10}              & \MC {2}{c}{7.62$\pm$0.10}               & \MC {2}{c}{...}                       \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J0705_PGC020125a.tex
%J0935-1348.tex
%J1001_PGC029033_se.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of ESO308-022, PGC020125 and 6dFJ0935-1348}
\label{t:Intens6}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{ESO308-022=J0639--4043   }    % \\ \hline
& \MC{2}{c}{PGC020125=J0705--5831    }    % \\ \hline
& \MC{2}{c}{6dFJ0935-1348=J0935--1348}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  1.284$\pm$ 0.074 &  1.239$\pm$ 0.078  &  2.427$\pm$ 0.172 &  2.372$\pm$ 0.190  &  1.819$\pm$ 0.191 &  1.765$\pm$ 0.406   \\
4101\ H$\delta$\                    &  0.142$\pm$ 0.018 &  0.219$\pm$ 0.031  &        ...        &        ...         &        ...        &        ...          \\
4340\ H$\gamma$\                    &  0.388$\pm$ 0.015 &  0.437$\pm$ 0.019  &  0.415$\pm$ 0.045 &  0.480$\pm$ 0.060  &  0.309$\pm$ 0.079 &  0.467$\pm$ 0.184   \\
4861\ H$\beta$\                     &  1.000$\pm$ 0.030 &  1.000$\pm$ 0.033  &  1.000$\pm$ 0.066 &  1.000$\pm$ 0.073  &  1.000$\pm$ 0.103 &  1.000$\pm$ 0.153   \\
4959\ [O\ {\sc iii}]\               &  0.728$\pm$ 0.027 &  0.681$\pm$ 0.027  &  0.055$\pm$ 0.042 &  0.051$\pm$ 0.042  &  0.480$\pm$ 0.061 &  0.383$\pm$ 0.061   \\
5007\ [O\ {\sc iii}]\               &  2.082$\pm$ 0.052 &  1.946$\pm$ 0.052  &  0.164$\pm$ 0.042 &  0.151$\pm$ 0.042  &  1.435$\pm$ 0.127 &  1.134$\pm$ 0.126   \\
6548\ [N\ {\sc ii}]\                &  0.030$\pm$ 0.022 &  0.027$\pm$ 0.021  &  0.053$\pm$ 0.053 &  0.046$\pm$ 0.050  &  0.056$\pm$ 0.134 &  0.037$\pm$ 0.111   \\
6563\ H$\alpha$\                    &  3.009$\pm$ 0.078 &  2.765$\pm$ 0.083  &  2.994$\pm$ 0.169 &  2.664$\pm$ 0.175  &  3.963$\pm$ 1.474 &  2.751$\pm$ 1.408   \\
6584\ [N\ {\sc ii}]\                &  0.099$\pm$ 0.026 &  0.090$\pm$ 0.025  &  0.193$\pm$ 0.065 &  0.170$\pm$ 0.062  &  0.159$\pm$ 0.090 &  0.105$\pm$ 0.077   \\
%                                                                                                                      
   &  &  &  &  & & \\                                                                                                  
C(H$\beta$)\ dex                    & \MC {2}{c}{0.04$\pm$0.03}              & \MC {2}{c}{0.07$\pm$0.07}               & \MC {2}{c}{0.26$\pm$0.48}              \\
EW(abs)\ \AA\                       & \MC {2}{c}{7.45$\pm$0.34}              & \MC {2}{c}{2.65$\pm$0.55}               & \MC {2}{c}{2.10$\pm$0.70}              \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{112.5$\pm$2.6}              & \MC {2}{c}{35.2$\pm$1.6}                & \MC {2}{c}{ 8.8$\pm$0.6}               \\
\hline                                                                                                                                                          
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{17320$\pm$2274}             & \MC {2}{c}{28082$\pm$2465}              & \MC {2}{c}{18931$\pm$2325}             \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{14755$\pm$512 }             & \MC {2}{c}{16862$\pm$9   }              & \MC {2}{c}{14959$\pm$66  }             \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{1.182$\pm$0.148}            & \MC {2}{c}{1.522$\pm$0.122}             & \MC {2}{c}{1.613$\pm$0.371}            \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{1.536$\pm$0.459}            & \MC {2}{c}{0.035$\pm$0.011}             & \MC {2}{c}{0.729$\pm$0.203}            \\
O/H($\times$10$^5$)\                & \MC {2}{c}{2.717$\pm$0.482}            & \MC {2}{c}{1.556$\pm$0.122}             & \MC {2}{c}{2.342$\pm$0.423}            \\
12+log(O/H)(s)\                     & \MC {2}{c}{7.34$\pm$0.04}              & \MC {2}{c}{7.18$\pm$0.06}               & \MC {2}{c}{7.28$\pm$0.07}              \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.46$\pm$0.12}              & \MC {2}{c}{7.22$\pm$0.10}               & \MC {2}{c}{7.39$\pm$0.12}              \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{7.53$\pm$0.10}              & \MC {2}{c}{...}                         & \MC {2}{c}{...}                        \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J1233_PGC041667a.tex
%J1236_PGC091215c.tex
%J1246_AGC227970.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC029033, PGC041667 and PGC091215}
\label{t:Intens7}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC029033=J10012--0814   }    % \\ \hline
& \MC{2}{c}{PGC041667=J1233--0031 }    % \\ \hline
& \MC{2}{c}{PGC091215=J1236+0136  }      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\               &  3.941$\pm$ 0.550 &  3.985$\pm$ 0.597    &  3.727$\pm$ 0.272 &  3.281$\pm$ 0.310  &  3.809$\pm$ 0.182 &  3.274$\pm$ 0.231  \\ 
4340\ H$\gamma$\                   &  0.431$\pm$ 0.125 &  0.471$\pm$ 0.230    &  0.364$\pm$ 0.051 &  0.467$\pm$ 0.099  &  0.224$\pm$ 0.034 &  0.475$\pm$ 0.118  \\
4861\ H$\beta$\                    &  1.000$\pm$ 0.139 &  1.000$\pm$ 0.323    &  1.000$\pm$ 0.086 &  1.000$\pm$ 0.115  &  1.000$\pm$ 0.046 &  1.000$\pm$ 0.067  \\ 
4959\ [O\ {\sc iii}]\              &  0.431$\pm$ 0.125 &  0.422$\pm$ 0.125    &  0.364$\pm$ 0.051 &  0.310$\pm$ 0.050  &  0.237$\pm$ 0.034 &  0.170$\pm$ 0.034  \\ 
5007\ [O\ {\sc iii}]\              &  1.294$\pm$ 0.160 &  1.263$\pm$ 0.160    &  1.106$\pm$ 0.090 &  0.944$\pm$ 0.090  &  0.757$\pm$ 0.036 &  0.538$\pm$ 0.036  \\ 
6548\ [N\ {\sc ii}]\               &        ...        &        ...           &  0.061$\pm$ 0.106 &  0.050$\pm$ 0.103  &  0.158$\pm$ 0.079 &  0.095$\pm$ 0.066  \\ 
6563\ H$\alpha$\                   &  2.980$\pm$ 0.323 &  2.839$\pm$ 0.431    &  3.303$\pm$ 0.281 &  2.824$\pm$ 0.306  &  4.257$\pm$ 0.183 &  2.727$\pm$ 0.177  \\ 
6584\ [N\ {\sc ii}]\               &        ...        &        ...           &  0.242$\pm$ 0.137 &  0.201$\pm$ 0.133  &  0.526$\pm$ 0.100 &  0.317$\pm$ 0.084  \\ 
%                                      
   &  &  &  &  & & \\                  
C(H$\beta$)\ dex                   & \MC {2}{c}{0.03$\pm$0.14}            & \MC {2}{c}{0.04$\pm$0.11}               & \MC {2}{c}{0.24$\pm$0.06}             \\
EW(abs)\ \AA\                      & \MC {2}{c}{0.10$\pm$0.32}            & \MC {2}{c}{2.70$\pm$0.89}               & \MC {2}{c}{1.95$\pm$0.07}             \\
EW(H$\beta$)\ \AA\                 & \MC {2}{c}{ 2.4$\pm$0.3}             & \MC {2}{c}{16.0$\pm$0.9}                & \MC {2}{c}{ 5.1$\pm$0.2}              \\  
\hline                                                                                                                                                          
$T_{\rm e}$(OIII)(K)\              & \MC {2}{c}{12039$\pm$1244}           & \MC {2}{c}{12970$\pm$1203}              & \MC {2}{c}{21226$\pm$2277}            \\
$T_{\rm e}$(OII)(K)\               & \MC {2}{c}{11866$\pm$1081}           & \MC {2}{c}{12622$\pm$909 }              & \MC {2}{c}{16020$\pm$567 }            \\
O$^{+}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{7.752$\pm$2.898}          & \MC {2}{c}{5.272$\pm$1.439}             & \MC {2}{c}{2.434$\pm$0.305}           \\
O$^{++}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{2.490$\pm$0.826}          & \MC {2}{c}{1.523$\pm$0.416}             & \MC {2}{c}{0.269$\pm$0.060}           \\
O/H($\times$10$^5$)\               & \MC {2}{c}{10.24$\pm$3.013}          & \MC {2}{c}{6.795$\pm$1.498}             & \MC {2}{c}{2.703$\pm$0.311}           \\
12+log(O/H)(s)\                    & \MC {2}{c}{...}                      & \MC {2}{c}{...}                         & \MC {2}{c}{7.36$\pm$0.05}             \\
12+log(O/H)(mse,c)\                & \MC {2}{c}{8.01$\pm$0.15}            & \MC {2}{c}{7.84$\pm$0.13}               & \MC {2}{c}{7.45$\pm$0.11:}            \\
%12+log(O/H)(PT05)\                 & \MC {2}{c}{...}                      & \MC {2}{c}{...}                         & \MC {2}{c}{...}                       \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J1249_UGC07983b.tex
%J1249_PGC1289726.tex
%J1250_AGC227973.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of AGC227970, UGC07983 and PGC1289726}
\label{t:Intens8}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{AGC227970=J1246+0422  }    % \\ \hline
& \MC{2}{c}{UGC07983=J1249+0350  }    % \\ \hline
& \MC{2}{c}{PGC1289726=J1249+0549}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  2.205$\pm$ 0.040 &  2.367$\pm$ 0.049   &  4.396$\pm$ 0.352 &  3.824$\pm$ 0.428  &  4.956$\pm$ 0.225 &  3.724$\pm$ 0.308  \\
3835\ H9\                           &  0.025$\pm$ 0.004 &  0.079$\pm$ 0.014   &        ...        &        ...         &        ...        &        ...         \\
3868\ [Ne\ {\sc iii}]\              &  0.182$\pm$ 0.005 &  0.193$\pm$ 0.006   &        ...        &        ...         &        ...        &        ...         \\
3889\ He\ {\sc i}\ +\ H8\           &  0.134$\pm$ 0.005 &  0.194$\pm$ 0.008   &        ...        &        ...         &        ...        &        ...         \\
3967\ [Ne\ {\sc iii}]\ +\ H7\       &  0.174$\pm$ 0.005 &  0.228$\pm$ 0.007   &        ...        &        ...         &        ...        &        ...         \\
4101\ H$\delta$\                    &  0.217$\pm$ 0.005 &  0.269$\pm$ 0.007   &        ...        &        ...         &        ...        &        ...         \\
4340\ H$\gamma$\                    &  0.427$\pm$ 0.013 &  0.471$\pm$ 0.015   &  0.243$\pm$ 0.056 &  0.478$\pm$ 0.171  &  0.096$\pm$ 0.026 &  0.469$\pm$ 0.275  \\
4363\ [O\ {\sc iii}]\               &  0.048$\pm$ 0.012 &  0.049$\pm$ 0.013   &        ...        &        ...         &        ...        &        ...         \\
4471\ He\ {\sc i}\                  &  0.027$\pm$ 0.003 &  0.027$\pm$ 0.003   &        ...        &        ...         &        ...        &        ...         \\
4861\ H$\beta$\                     &  1.000$\pm$ 0.020 &  1.000$\pm$ 0.021   &  1.000$\pm$ 0.089 &  1.000$\pm$ 0.124  &  1.000$\pm$ 0.057 &  1.000$\pm$ 0.100  \\
4959\ [O\ {\sc iii}]\               &  0.835$\pm$ 0.017 &  0.805$\pm$ 0.017   &  0.694$\pm$ 0.070 &  0.524$\pm$ 0.069  &  0.638$\pm$ 0.042 &  0.385$\pm$ 0.042  \\
5007\ [O\ {\sc iii}]\               &  2.519$\pm$ 0.050 &  2.422$\pm$ 0.049   &  2.297$\pm$ 0.162 &  1.728$\pm$ 0.160  &  2.214$\pm$ 0.107 &  1.325$\pm$ 0.106  \\
6300\ [O\ {\sc i}]\                 &  0.046$\pm$ 0.007 &  0.041$\pm$ 0.007   &        ...        &        ...         &        ...        &        ...         \\
6312\ [S\ {\sc iii}]\               &  0.020$\pm$ 0.007 &  0.017$\pm$ 0.007   &        ...        &        ...         &        ...        &        ...         \\
6548\ [N\ {\sc ii}]\                &  0.035$\pm$ 0.008 &  0.031$\pm$ 0.007   &  0.027$\pm$ 0.063 &  0.018$\pm$ 0.055  &  0.170$\pm$ 0.118 &  0.083$\pm$ 0.095  \\
6563\ H$\alpha$\                    &  3.180$\pm$ 0.064 &  2.792$\pm$ 0.063   &  4.081$\pm$ 0.291 &  2.846$\pm$ 0.290  &  5.129$\pm$ 0.276 &  2.772$\pm$ 0.266  \\
6584\ [N\ {\sc ii}]\                &  0.107$\pm$ 0.012 &  0.094$\pm$ 0.011   &  0.117$\pm$ 0.081 &  0.078$\pm$ 0.071  &  0.494$\pm$ 0.134 &  0.242$\pm$ 0.108  \\
%                                   
   &  &  &  &  & & \\               
C(H$\beta$)\ dex                    & \MC {2}{c}{0.14$\pm$0.03}               & \MC {2}{c}{0.18$\pm$0.09}              & \MC {2}{c}{0.29$\pm$0.07}              \\
EW(abs)\ \AA\                       & \MC {2}{c}{2.80$\pm$0.17}               & \MC {2}{c}{2.15$\pm$0.25}              & \MC {2}{c}{2.15$\pm$0.06}              \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{97.4$\pm$1.4}                & \MC {2}{c}{6.92$\pm$0.41}               & \MC {2}{c}{ 3.4$\pm$0.1}               \\
\hline                                                                                                                                                              
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{15323$\pm$1870}              & \MC {2}{c}{12108$\pm$1201}             & \MC {2}{c}{17062$\pm$2275}             \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{14063$\pm$876 }              & \MC {2}{c}{11925$\pm$1034}             & \MC {2}{c}{14693$\pm$583 }             \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{2.633$\pm$0.536}             & \MC {2}{c}{7.557$\pm$2.585}            & \MC {2}{c}{3.601$\pm$0.539}            \\
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{2.523$\pm$0.764}             & \MC {2}{c}{3.335$\pm$1.015}            & \MC {2}{c}{1.034$\pm$0.324}            \\
O/H($\times$10$^5$)\                & \MC {2}{c}{5.156$\pm$0.934}             & \MC {2}{c}{10.89$\pm$2.777}            & \MC {2}{c}{4.635$\pm$0.628}            \\
12+log(O/H)(d)\                     & \MC {2}{c}{7.71$\pm$0.08}               & \MC {2}{c}{...}                        & \MC {2}{c}{...}                        \\
%12+log(O/H)(s)\                     & \MC {2}{c}{...}                         & \MC {2}{c}{...}                        & \MC {2}{c}{...}                        \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.79$\pm$0.11}               & \MC {2}{c}{8.03$\pm$0.14}              & \MC {2}{c}{7.68$\pm$0.11}              \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{7.83$\pm$0.10}               & \MC {2}{c}{...}                        & \MC {2}{c}{...}                        \\
\MC{3}{l}{~~} \                                                                                                        
\end{tabular}                                                                                                           
 }
\end{table*}


%J1253_PGC1264260.tex
%J1256_UGC08055.tex
%J1259_PGC044681a.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of AGC227973, PGC1264260 and UGC08055}
\label{t:Intens9}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{AGC227973=J1250+0520 }    % \\ \hline
& \MC{2}{c}{PGC1264260=J1253+0409 }    % \\ \hline
& \MC{2}{c}{UGC08055=J1256+0348   }      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                &  0.977$\pm$ 0.090 &  0.977$\pm$ 0.102  &  3.402$\pm$ 0.072 &  3.180$\pm$ 0.086  &  2.578$\pm$ 0.070 &  2.637$\pm$ 0.081    \\ 
3868\ [Ne\ {\sc iii}]\              &        ...        &        ...         &        ...        &        ...         &  0.169$\pm$ 0.015 &  0.171$\pm$ 0.016    \\ 
3889\ He\ {\sc i}\ +\ H8\           &        ...        &        ...         &        ...        &        ...         &  0.083$\pm$ 0.012 &  0.172$\pm$ 0.033    \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\       &        ...        &        ...         &        ...        &        ...         &  0.123$\pm$ 0.015 &  0.205$\pm$ 0.030    \\ 
4101\ H$\delta$\                    &  0.263$\pm$ 0.032 &  0.342$\pm$ 0.048  &  0.074$\pm$ 0.006 &  0.270$\pm$ 0.031  &  0.179$\pm$ 0.011 &  0.250$\pm$ 0.018    \\ 
4340\ H$\gamma$\                    &  0.384$\pm$ 0.033 &  0.460$\pm$ 0.046  &  0.339$\pm$ 0.035 &  0.480$\pm$ 0.062  &  0.420$\pm$ 0.039 &  0.475$\pm$ 0.048    \\ 
4363\ [O\ {\sc iii}]\               &        ...        &        ...         &  0.049$\pm$ 0.025 &  0.043$\pm$ 0.026  &        ...        &        ...           \\ 
4861\ H$\beta$\                     &  1.000$\pm$ 0.053 &  1.000$\pm$ 0.060  &  1.000$\pm$ 0.024 &  1.000$\pm$ 0.029  &  1.000$\pm$ 0.028 &  1.000$\pm$ 0.030    \\ 
4959\ [O\ {\sc iii}]\               &  0.256$\pm$ 0.032 &  0.231$\pm$ 0.031  &  0.576$\pm$ 0.017 &  0.485$\pm$ 0.017  &  0.642$\pm$ 0.019 &  0.606$\pm$ 0.019    \\ 
5007\ [O\ {\sc iii}]\               &  0.759$\pm$ 0.042 &  0.685$\pm$ 0.041  &  1.675$\pm$ 0.033 &  1.408$\pm$ 0.033  &  2.069$\pm$ 0.051 &  1.949$\pm$ 0.051    \\ 
6548\ [N\ {\sc ii}]\                &  0.007$\pm$ 0.045 &  0.006$\pm$ 0.041  &  0.055$\pm$ 0.027 &  0.042$\pm$ 0.024  &  0.049$\pm$ 0.028 &  0.043$\pm$ 0.026    \\ 
6563\ H$\alpha$\                    &  3.241$\pm$ 0.166 &  2.716$\pm$ 0.166  &  3.460$\pm$ 0.075 &  2.749$\pm$ 0.077  &  3.181$\pm$ 0.085 &  2.810$\pm$ 0.086    \\ 
6584\ [N\ {\sc ii}]\                &  0.053$\pm$ 0.068 &  0.043$\pm$ 0.061  &  0.168$\pm$ 0.031 &  0.129$\pm$ 0.028  &  0.156$\pm$ 0.032 &  0.137$\pm$ 0.030    \\ 
%                                                                                                                       
   &  &  &  &  & & \\                                                                                                   
C(H$\beta$)\ dex                    & \MC {2}{c}{0.13$\pm$0.07}            & \MC {2}{c}{0.14$\pm$0.03}              & \MC {2}{c}{0.10$\pm$0.03}                \\
EW(abs)\ \AA\                       & \MC {2}{c}{2.05$\pm$0.23}            & \MC {2}{c}{2.35$\pm$0.04}              & \MC {2}{c}{1.45$\pm$0.17}                \\
EW(H$\beta$)\ \AA\                  & \MC {2}{c}{21.0$\pm$0.7}             & \MC {2}{c}{13.2$\pm$0.2}               & \MC {2}{c}{27.3$\pm$0.6}                 \\  
\hline                                                                                                                                                             
$T_{\rm e}$(OIII)(K)\               & \MC {2}{c}{22082$\pm$2307}           & \MC {2}{c}{18780$\pm$6534}             & \MC {2}{c}{13997$\pm$1160}               \\
$T_{\rm e}$(OII)(K)\                & \MC {2}{c}{16220$\pm$502 }           & \MC {2}{c}{14954$\pm$306 }             & \MC {2}{c}{13334$\pm$731 }               \\
O$^{+}$/H$^{+}$($\times$10$^5$)\    & \MC {2}{c}{0.700$\pm$0.097}          & \MC {2}{c}{2.910$\pm$0.200}            & \MC {2}{c}{3.501$\pm$0.661}              \\ 
O$^{++}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{0.322$\pm$0.067}          & \MC {2}{c}{0.926$\pm$0.691}            & \MC {2}{c}{2.519$\pm$0.556}              \\ 
O/H($\times$10$^5$)\                & \MC {2}{c}{1.023$\pm$0.118}          & \MC {2}{c}{3.836$\pm$0.719}            & \MC {2}{c}{6.020$\pm$0.864}              \\ 
12+log(O/H)(d)\                     & \MC {2}{c}{...}                      & \MC {2}{c}{7.58$\pm$0.08}              & \MC {2}{c}{...}                          \\
12+log(O/H)(s)\                     & \MC {2}{c}{7.05$\pm$0.06}            & \MC {2}{c}{7.46$\pm$0.04}              & \MC {2}{c}{...}                          \\
12+log(O/H)(mse,c)\                 & \MC {2}{c}{7.01$\pm$0.10}            & \MC {2}{c}{...}                        & \MC {2}{c}{7.79$\pm$0.11}                \\
12+log(O/H)(PT05)\                  & \MC {2}{c}{...}                      & \MC {2}{c}{...}                        & \MC {2}{c}{7.79$\pm$0.10}                \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J1430_AGC716018.tex
%J1449_AGC249197.tex
%J1738_HIPASSJ1738_1.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC044681, AGC716018 and AGC249197}
\label{t:Intens10}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC044681=J1259--1924 }    % \\ \hline
& \MC{2}{c}{AGC716018=J1430+0709  }    % \\ \hline
& \MC{2}{c}{AGC249197=J1449+0956  }      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\               &  2.175$\pm$ 0.370 &  2.505$\pm$ 0.443   &  3.522$\pm$ 0.523 &  2.762$\pm$ 0.591  &  4.000$\pm$ 0.407 &  3.054$\pm$ 0.489   \\
4101\ H$\delta$\                   &  ...              &  ...                &  0.071$\pm$ 0.045 &  0.318$\pm$ 0.356  &  ...              &  ...                 \\
4340\ H$\gamma$\                   &  0.450$\pm$ 0.087 &  0.481$\pm$ 0.187   &  0.216$\pm$ 0.082 &  0.437$\pm$ 0.259  &  0.238$\pm$ 0.053 &  0.480$\pm$ 0.438   \\
4861\ H$\beta$\                    &  1.000$\pm$ 0.141 &  1.000$\pm$ 0.200   &  1.000$\pm$ 0.160 &  1.000$\pm$ 0.218  &  1.000$\pm$ 0.135 &  1.000$\pm$ 0.440   \\
4959\ [O\ {\sc iii}]\              &  0.325$\pm$ 0.060 &  0.320$\pm$ 0.059   &  1.544$\pm$ 0.202 &  1.157$\pm$ 0.202  &  0.381$\pm$ 0.060 &  0.264$\pm$ 0.060   \\
5007\ [O\ {\sc iii}]\              &  1.000$\pm$ 0.125 &  0.980$\pm$ 0.123   &  3.341$\pm$ 0.390 &  2.500$\pm$ 0.389  &  1.333$\pm$ 0.159 &  0.922$\pm$ 0.158   \\
6548\ [N\ {\sc ii}]\               &        ...        &        ...          &  0.080$\pm$ 0.219 &  0.057$\pm$ 0.209  &  0.048$\pm$ 0.095 &  0.030$\pm$ 0.087   \\
6563\ H$\alpha$\                   &  3.225$\pm$ 0.331 &  2.748$\pm$ 0.317   &  3.688$\pm$ 0.556 &  2.820$\pm$ 0.615  &  4.000$\pm$ 0.449 &  2.747$\pm$ 0.552   \\
6584\ [N\ {\sc ii}]\               &        ...        &        ...          &  0.359$\pm$ 0.285 &  0.258$\pm$ 0.273  &  0.191$\pm$ 0.144 &  0.121$\pm$ 0.131   \\
%                                   
   &  &  &  &  & & \\               
C(H$\beta$)\ dex                   & \MC {2}{c}{0.20$\pm$0.13}               & \MC {2}{c}{0.06$\pm$0.20}              & \MC {2}{c}{0.12$\pm$0.15}               \\
EW(abs)\ \AA\                      & \MC {2}{c}{0.10$\pm$3.47}               & \MC {2}{c}{1.10$\pm$0.11}              & \MC {2}{c}{1.60$\pm$1.46}               \\
EW(H$\beta$)\ \AA\                 & \MC {2}{c}{24.8$\pm$2.3}                & \MC {2}{c}{ 3.3$\pm$0.4}               & \MC {2}{c}{ 3.7$\pm$0.3}                \\
\hline                                                                                                                                                              
$T_{\rm e}$(OIII)(K)\              & \MC {2}{c}{18959$\pm$2301}              & \MC {2}{c}{13128$\pm$1294}             & \MC {2}{c}{18946$\pm$2303}              \\
$T_{\rm e}$(OII)(K)\               & \MC {2}{c}{14960$\pm$58  }              & \MC {2}{c}{12740$\pm$953 }             & \MC {2}{c}{14960$\pm$61  }              \\
O$^{+}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{2.290$\pm$0.406}             & \MC {2}{c}{4.295$\pm$1.460}            & \MC {2}{c}{2.791$\pm$0.448}             \\
O$^{++}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{0.623$\pm$0.174}             & \MC {2}{c}{4.292$\pm$1.286}            & \MC {2}{c}{0.570$\pm$0.168}             \\
O/H($\times$10$^5$)\               & \MC {2}{c}{2.913$\pm$0.441}             & \MC {2}{c}{8.587$\pm$1.946}            & \MC {2}{c}{3.361$\pm$0.479}             \\
12+log(O/H)(s)\                    & \MC {2}{c}{7.34$\pm$0.07}               & \MC {2}{c}{}                           & \MC {2}{c}{7.39$\pm$0.06}               \\
12+log(O/H)(mse,c)\                & \MC {2}{c}{7.48$\pm$0.11:}              & \MC {2}{c}{7.93$\pm$0.14}              & \MC {2}{c}{7.53$\pm$0.11:}              \\
12+log(O/H)(PT05)\                 & \MC {2}{c}{...}                         & \MC {2}{c}{7.96$\pm$0.10}              & \MC {2}{c}{...}                         \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J2026_PGC408791a.tex
%J2108_PGC129680b.tex
%J2139_PGC1016598E.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of HIPASSJ1738-57, PGC408791 and PGC129680}
\label{t:Intens11}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{HIPASSJ1738-57=J1738--5715}    % \\ \hline
& \MC{2}{c}{PGC408791=J2026--5529 }    % \\ \hline
& \MC{2}{c}{PGC129680=J2108--4719 }      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\              &  2.025$\pm$ 0.031 &  2.025$\pm$ 0.044  &  2.487$\pm$ 0.206 &  2.673$\pm$ 0.262  &  3.510$\pm$ 0.270 &  3.000$\pm$ 0.394   \\
3868\ [Ne\ {\sc iii}]\            &  0.245$\pm$ 0.026 &  0.241$\pm$ 0.029  &        ...        &        ...         &  0.292$\pm$ 0.076 &  0.241$\pm$ 0.097   \\
3967\ [Ne\ {\sc iii}]\ +\ H7\     &  0.077$\pm$ 0.010 &  0.222$\pm$ 0.040  &        ...        &        ...         &        ...        &        ...          \\
4101\ H$\delta$\                  &  0.127$\pm$ 0.013 &  0.273$\pm$ 0.037  &  0.035$\pm$ 0.035 &  0.253$\pm$ 0.477  &        ...        &        ...          \\
4340\ H$\gamma$\                  &  0.346$\pm$ 0.028 &  0.458$\pm$ 0.044  &  0.348$\pm$ 0.064 &  0.483$\pm$ 0.191  &  0.082$\pm$ 0.033 &  0.463$\pm$ 0.382   \\
4363\ [O\ {\sc iii}]\             &  0.045$\pm$ 0.023 &  0.042$\pm$ 0.024  &        ...        &        ...         &        ...        &        ...          \\
4861\ H$\beta$\                   &  1.000$\pm$ 0.018 &  1.000$\pm$ 0.023  &  1.000$\pm$ 0.086 &  1.000$\pm$ 0.158  &  1.000$\pm$ 0.087 &  1.000$\pm$ 0.143   \\
4959\ [O\ {\sc iii}]\             &  0.945$\pm$ 0.015 &  0.833$\pm$ 0.015  &  0.470$\pm$ 0.067 &  0.409$\pm$ 0.067  &  1.881$\pm$ 0.142 &  1.208$\pm$ 0.140   \\
5007\ [O\ {\sc iii}]\             &  2.852$\pm$ 0.042 &  2.504$\pm$ 0.042  &  1.417$\pm$ 0.106 &  1.226$\pm$ 0.104  &  5.646$\pm$ 0.368 &  3.593$\pm$ 0.360   \\
6548\ [N\ {\sc ii}]\              &  0.033$\pm$ 0.013 &  0.026$\pm$ 0.011  &        ...        &        ...         &  0.148$\pm$ 0.255 &  0.073$\pm$ 0.193   \\
6563\ H$\alpha$\                  &  3.501$\pm$ 0.096 &  2.808$\pm$ 0.094  &  3.756$\pm$ 0.242 &  2.763$\pm$ 0.226  &  5.375$\pm$ 0.491 &  2.838$\pm$ 0.433   \\
6584\ [N\ {\sc ii}]\              &  0.104$\pm$ 0.025 &  0.081$\pm$ 0.022  &        ...        &        ...         &  0.399$\pm$ 0.289 &  0.196$\pm$ 0.218   \\
%                                                                                                                      
   &  &  &  &  & & \\                                                                                                  
C(H$\beta$)\ dex                   & \MC {2}{c}{0.17$\pm$0.04}             & \MC {2}{c}{0.27$\pm$0.08}              & \MC {2}{c}{0.38$\pm$0.12}               \\
EW(abs)\ \AA\                      & \MC {2}{c}{2.20$\pm$0.15}             & \MC {2}{c}{2.40$\pm$2.22}              & \MC {2}{c}{1.00$\pm$0.07}               \\
EW(H$\beta$)\ \AA\                 & \MC {2}{c}{17.7$\pm$0.2}              & \MC {2}{c}{18.1$\pm$1.0}               & \MC {2}{c}{ 1.9$\pm$0.1}                \\
\hline                                                                                                                                                        
$T_{\rm e}$(OIII)(K)\              & \MC {2}{c}{14120$\pm$3453}            & \MC {2}{c}{17902$\pm$2279}             & \MC {2}{c}{12512$\pm$1208}              \\
$T_{\rm e}$(OII)(K)\               & \MC {2}{c}{13410$\pm$2125}            & \MC {2}{c}{14865$\pm$351 }             & \MC {2}{c}{12264$\pm$980 }              \\
O$^{+}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{2.637$\pm$1.414}           & \MC {2}{c}{2.471$\pm$0.304}            & \MC {2}{c}{5.348$\pm$1.708}             \\
O$^{++}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{3.215$\pm$2.073}           & \MC {2}{c}{0.888$\pm$0.259}            & \MC {2}{c}{6.458$\pm$1.877}             \\
O/H($\times$10$^5$)\               & \MC {2}{c}{5.852$\pm$2.509}           & \MC {2}{c}{3.358$\pm$0.400}            & \MC {2}{c}{11.81$\pm$2.537}             \\
12+log(O/H)(d)\                    & \MC {2}{c}{7.77$\pm$0.19}             & \MC {2}{c}{...}                        & \MC {2}{c}{...}                         \\
12+log(O/H)(s)\                    & \MC {2}{c}{...}                       & \MC {2}{c}{7.39$\pm$0.05}              & \MC {2}{c}{...}                         \\
12+log(O/H)(mse,c)\                & \MC {2}{c}{7.72$\pm$0.11}             & \MC {2}{c}{7.54$\pm$0.11}              & \MC {2}{c}{8.07$\pm$0.13}               \\
12+log(O/H)(PT05)\                 & \MC {2}{c}{7.76$\pm$0.10}             & \MC {2}{c}{...}                        & \MC {2}{c}{8.15$\pm$0.10}               \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J2221_ESO289-020.tex
%J2222_ESO238-005.tex
%J2242_PGC1028063.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC1016598, ESO289-020 and ESO238-005}
\label{t:Intens12}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC1016598=J2139--0734}    % \\ \hline
& \MC{2}{c}{ESO289-020=J2221--4540}    % \\ \hline
& \MC{2}{c}{ESO238-005=J2222--4824}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\               &  1.117$\pm$ 0.192 &  0.909$\pm$ 0.193 &  2.006$\pm$ 0.084 &  1.554$\pm$ 0.092   &  2.169$\pm$ 0.059 &  1.959$\pm$ 0.064    \\ 
3868\ [Ne\ {\sc iii}]\             &        ...        &        ...        &  0.324$\pm$ 0.032 &  0.250$\pm$ 0.033   &  0.172$\pm$ 0.028 &  0.155$\pm$ 0.028    \\ 
4101\ H$\delta$\                   &  0.101$\pm$ 0.050 &  0.246$\pm$ 0.254 &        ...        &        ...          &  0.114$\pm$ 0.028 &  0.256$\pm$ 0.084    \\
4340\ H$\gamma$\                   &  0.167$\pm$ 0.051 &  0.268$\pm$ 0.181 &  0.233$\pm$ 0.067 &  0.475$\pm$ 0.214   &  0.381$\pm$ 0.018 &  0.475$\pm$ 0.031    \\
4861\ H$\beta$\                    &  1.000$\pm$ 0.071 &  1.000$\pm$ 0.217 &  1.000$\pm$ 0.039 &  1.000$\pm$ 0.057   &  1.000$\pm$ 0.027 &  1.000$\pm$ 0.034    \\
4959\ [O\ {\sc iii}]\              &  0.717$\pm$ 0.076 &  0.583$\pm$ 0.076 &  0.961$\pm$ 0.034 &  0.727$\pm$ 0.034   &  0.542$\pm$ 0.020 &  0.483$\pm$ 0.020    \\ 
5007\ [O\ {\sc iii}]\              &  2.133$\pm$ 0.126 &  1.736$\pm$ 0.126 &  2.618$\pm$ 0.079 &  1.981$\pm$ 0.079   &  1.645$\pm$ 0.040 &  1.468$\pm$ 0.040    \\ 
6548\ [N\ {\sc ii}]\               &        ...        &        ...        &  0.058$\pm$ 0.061 &  0.043$\pm$ 0.059   &  0.058$\pm$ 0.036 &  0.051$\pm$ 0.036    \\ 
6563\ H$\alpha$\                   &  3.167$\pm$ 0.166 &  2.749$\pm$ 0.266 &  3.479$\pm$ 0.136 &  2.779$\pm$ 0.157   &  3.046$\pm$ 0.082 &  2.760$\pm$ 0.091    \\
6584\ [N\ {\sc ii}]\               &        ...        &        ...        &  0.182$\pm$ 0.070 &  0.135$\pm$ 0.068   &  0.179$\pm$ 0.039 &  0.158$\pm$ 0.038    \\ 
%                                                                                                                      
   &  &  &  &  & & \\                                                                                                  
C(H$\beta$)\ dex                  & \MC {2}{c}{0.00$\pm$0.07}              & \MC {2}{c}{0.03$\pm$0.05}               & \MC {2}{c}{0.01$\pm$0.04}                \\
EW(abs)\ \AA\                     & \MC {2}{c}{6.80$\pm$5.90}              & \MC {2}{c}{3.55$\pm$0.26}               & \MC {2}{c}{3.50$\pm$0.39}                \\
EW(H$\beta$)\ \AA\                & \MC {2}{c}{29.7$\pm$1.4}               & \MC {2}{c}{11.1$\pm$0.3}                & \MC {2}{c}{29.4$\pm$0.6}                 \\  
\hline                                                                                                                                                            
$T_{\rm e}$(OIII)(K)\             & \MC {2}{c}{18423$\pm$2327}             & \MC {2}{c}{16226$\pm$1169}              & \MC {2}{c}{17687$\pm$2271}               \\
$T_{\rm e}$(OII)(K)\              & \MC {2}{c}{14929$\pm$210 }             & \MC {2}{c}{14436$\pm$419 }              & \MC {2}{c}{14830$\pm$409 }               \\
O$^{+}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{0.836$\pm$0.181}            & \MC {2}{c}{1.589$\pm$0.174}             & \MC {2}{c}{1.840$\pm$0.170}              \\ 
O$^{++}$/H$^{+}$($\times$10$^5$)\ & \MC {2}{c}{1.182$\pm$0.333}            & \MC {2}{c}{1.842$\pm$0.321}             & \MC {2}{c}{1.088$\pm$0.313}              \\ 
O/H($\times$10$^5$)\              & \MC {2}{c}{2.018$\pm$0.379}            & \MC {2}{c}{3.431$\pm$0.365}             & \MC {2}{c}{2.928$\pm$0.356}              \\ 
12+log(O/H)(s)\                   & \MC {2}{c}{7.26$\pm$0.05}              & \MC {2}{c}{7.38$\pm$0.05}               & \MC {2}{c}{7.35$\pm$0.04}                \\
12+log(O/H)(mse,c)\               & \MC {2}{c}{7.33$\pm$0.12}              & \MC {2}{c}{7.55$\pm$0.10}               & \MC {2}{c}{7.49$\pm$0.11}                \\
12+log(O/H)(PT05)\                & \MC {2}{c}{7.41$\pm$0.10}              & \MC {2}{c}{7.61$\pm$0.10}               & \MC {2}{c}{...}                          \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}



%J2326_ESO347-017a.tex
%J2341_PGC3192333.tex
%J2341_PGC680341.tex
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC1028063, ESO347-017 and PGC3192333}
\label{t:Intens13}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC1028063=J2242--0650}    % \\ \hline
& \MC{2}{c}{ESO347-017=J2326--3720}    % \\ \hline
& \MC{2}{c}{PGC3192333=J2341--3530}      \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\           &  1.982$\pm$ 0.056 &  1.966$\pm$ 0.065 &  2.521$\pm$ 0.065 &  2.715$\pm$ 0.081  &  1.422$\pm$ 0.091 &  1.307$\pm$ 0.093    \\ 
3868\ [Ne\ {\sc iii}]\         &  0.284$\pm$ 0.012 &  0.280$\pm$ 0.013 &  0.234$\pm$ 0.009 &  0.248$\pm$ 0.010  &        ...        &        ...           \\ 
3889\ He\ {\sc i}\ +\ H8\      &  0.080$\pm$ 0.011 &  0.188$\pm$ 0.034 &  0.133$\pm$ 0.007 &  0.207$\pm$ 0.013  &        ...        &        ...           \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\  &  0.117$\pm$ 0.006 &  0.216$\pm$ 0.015 &  0.140$\pm$ 0.006 &  0.213$\pm$ 0.011  &        ...        &        ...           \\ 
4101\ H$\delta$\               &  0.189$\pm$ 0.009 &  0.273$\pm$ 0.016 &  0.202$\pm$ 0.006 &  0.265$\pm$ 0.010  &  0.234$\pm$ 0.033 &  0.294$\pm$ 0.049    \\
4340\ H$\gamma$\               &  0.408$\pm$ 0.022 &  0.468$\pm$ 0.028 &  0.413$\pm$ 0.013 &  0.468$\pm$ 0.016  &  0.377$\pm$ 0.041 &  0.427$\pm$ 0.052    \\
4363\ [O\ {\sc iii}]\          &  0.067$\pm$ 0.017 &  0.064$\pm$ 0.017 &  0.050$\pm$ 0.003 &  0.051$\pm$ 0.004  &  0.033$\pm$ 0.013 &  0.030$\pm$ 0.013    \\  
4471\ He\ {\sc i}\             &  0.024$\pm$ 0.005 &  0.023$\pm$ 0.005 &  0.025$\pm$ 0.003 &  0.025$\pm$ 0.003  &        ...        &        ...           \\ 
4861\ H$\beta$\                &  1.000$\pm$ 0.035 &  1.000$\pm$ 0.038 &  1.000$\pm$ 0.032 &  1.000$\pm$ 0.034  &  1.000$\pm$ 0.046 &  1.000$\pm$ 0.051    \\
4959\ [O\ {\sc iii}]\          &  1.216$\pm$ 0.040 &  1.130$\pm$ 0.040 &  0.990$\pm$ 0.031 &  0.944$\pm$ 0.031  &  0.351$\pm$ 0.034 &  0.322$\pm$ 0.034    \\  
5007\ [O\ {\sc iii}]\          &  3.648$\pm$ 0.112 &  3.385$\pm$ 0.112 &  2.952$\pm$ 0.094 &  2.804$\pm$ 0.093  &  1.046$\pm$ 0.047 &  0.961$\pm$ 0.047    \\  
6300\ [O\ {\sc i}]\            &  0.021$\pm$ 0.003 &  0.018$\pm$ 0.003 &  0.049$\pm$ 0.003 &  0.043$\pm$ 0.002  &        ...        &        ...           \\ 
6312\ [S\ {\sc iii}]\          &  0.016$\pm$ 0.002 &  0.014$\pm$ 0.002 &  0.010$\pm$ 0.002 &  0.009$\pm$ 0.002  &        ...        &        ...           \\ 
6364\ [O\ {\sc i}]\            &        ...        &        ...        &  0.013$\pm$ 0.002 &  0.011$\pm$ 0.002  &        ...        &        ...           \\ 
6548\ [N\ {\sc ii}]\           &  0.032$\pm$ 0.012 &  0.028$\pm$ 0.011 &  0.046$\pm$ 0.008 &  0.039$\pm$ 0.007  &        ...        &        ...           \\ 
6563\ H$\alpha$\               &  3.153$\pm$ 0.093 &  2.798$\pm$ 0.097 &  3.270$\pm$ 0.100 &  2.804$\pm$ 0.097  &  2.922$\pm$ 0.111 &  2.744$\pm$ 0.124    \\ 
6584\ [N\ {\sc ii}]\           &  0.097$\pm$ 0.016 &  0.085$\pm$ 0.015 &  0.139$\pm$ 0.017 &  0.118$\pm$ 0.015  &        ...        &        ...           \\ 
%                                   
   &  &  &  &  & & \\                                                               
C(H$\beta$)\ dex                  & \MC {2}{c}{0.09$\pm$0.04}          & \MC {2}{c}{0.16$\pm$0.04}         & \MC {2}{c}{0.00$\pm$0.05}                 \\
EW(abs)\ \AA\                     & \MC {2}{c}{2.30$\pm$0.18}          & \MC {2}{c}{2.40$\pm$0.17}         & \MC {2}{c}{2.10$\pm$0.26}                 \\
EW(H$\beta$)\ \AA\                & \MC {2}{c}{32.6$\pm$0.8}           & \MC {2}{c}{60.0$\pm$1.4}          & \MC {2}{c}{23.9$\pm$0.8}                  \\  
\hline                                                                                                                                                  
$T_{\rm e}$(OIII)(K)\             & \MC {2}{c}{14816$\pm$1780}         & \MC {2}{c}{14531$\pm$486 }        & \MC {2}{c}{19062$\pm$4841}                \\
$T_{\rm e}$(OII)(K)\              & \MC {2}{c}{13810$\pm$944 }         & \MC {2}{c}{13653$\pm$274 }        & \MC {2}{c}{14962$\pm$60  }                \\
O$^{+}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{2.321$\pm$0.530}        & \MC {2}{c}{3.329$\pm$0.244}       & \MC {2}{c}{1.194$\pm$0.086}               \\ 
O$^{++}$/H$^{+}$($\times$10$^5$)\ & \MC {2}{c}{3.840$\pm$1.177}        & \MC {2}{c}{3.350$\pm$0.302}       & \MC {2}{c}{0.608$\pm$0.329}               \\ 
O/H($\times$10$^5$)\              & \MC {2}{c}{6.162$\pm$1.291}        & \MC {2}{c}{6.680$\pm$0.388}       & \MC {2}{c}{1.802$\pm$0.340}               \\ 
12+log(O/H)(d)\                   & \MC {2}{c}{7.79$\pm$0.09}          & \MC {2}{c}{7.82$\pm$0.03}         & \MC {2}{c}{7.26$\pm$0.08}                 \\
12+log(O/H)(s)\                   & \MC {2}{c}{...}                    & \MC {2}{c}{...}                   & \MC {2}{c}{7.18$\pm$0.05}                 \\
12+log(O/H)(mse,c)\               & \MC {2}{c}{7.83$\pm$0.11}          & \MC {2}{c}{7.91$\pm$0.11}         & \MC {2}{c}{7.23$\pm$0.10}                 \\
12+log(O/H)(PT05)\                & \MC {2}{c}{7.87$\pm$0.10}          & \MC {2}{c}{7.96$\pm$0.10}         & \MC {2}{c}{...}                           \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


%J2349_ESO348-009.tex
%J2352_ESO149-003.tex
%
\begin{table*}            
\centering{
\caption{Line intensities and derived parameters of PGC680341, ESO348-009 and ESO149-003}
\label{t:Intens14}
\begin{tabular}{lcccccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC680341=J2341--3308 }    % \\ \hline
& \MC{2}{c}{ESO348-009=J2349--3746}    % \\ \hline
& \MC{2}{c}{ESO149-003=J2352--5234}     \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion   & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O{\sc ii}]\               &  1.664$\pm$ 0.034 &  1.484$\pm$ 0.039  &  3.100$\pm$ 0.156 &  2.946$\pm$ 0.186 &  1.704$\pm$ 0.065 &  2.277$\pm$ 0.095     \\ 
3868\ [Ne\ {\sc iii}]\           &        ...        &        ...         &  0.240$\pm$ 0.064 &  0.226$\pm$ 0.068 &  0.200$\pm$ 0.012 &  0.257$\pm$ 0.016     \\ 
3889\ He\ {\sc i}\ +\ H8\        &        ...        &        ...         &  0.077$\pm$ 0.040 &  0.250$\pm$ 0.185 &  0.152$\pm$ 0.011 &  0.195$\pm$ 0.016     \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\    &        ...        &        ...         &        ...        &        ...        &  0.169$\pm$ 0.008 &  0.212$\pm$ 0.013     \\ 
4101\ H$\delta$\                 &  0.147$\pm$ 0.010 &  0.286$\pm$ 0.025  &  0.217$\pm$ 0.028 &  0.338$\pm$ 0.056 &  0.224$\pm$ 0.010 &  0.271$\pm$ 0.015     \\ 
4340\ H$\gamma$\                 &  0.369$\pm$ 0.012 &  0.467$\pm$ 0.019  &  0.337$\pm$ 0.028 &  0.447$\pm$ 0.046 &  0.448$\pm$ 0.019 &  0.508$\pm$ 0.023     \\ 
4363\ [O\ {\sc iii}]\            &  0.059$\pm$ 0.008 &  0.052$\pm$ 0.008  &        ...        &        ...        &  0.047$\pm$ 0.004 &  0.053$\pm$ 0.004     \\ 
4471\ He\ {\sc i}\               &        ...        &        ...         &        ...        &        ...        &  0.030$\pm$ 0.004 &  0.032$\pm$ 0.004     \\ 
4861\ H$\beta$\                  &  1.000$\pm$ 0.022 &  1.000$\pm$ 0.025  &  1.000$\pm$ 0.061 &  1.000$\pm$ 0.071 &  1.000$\pm$ 0.052 &  1.000$\pm$ 0.052     \\ 
4959\ [O\ {\sc iii}]\            &  0.603$\pm$ 0.015 &  0.534$\pm$ 0.015  &  0.430$\pm$ 0.035 &  0.380$\pm$ 0.035 &  0.822$\pm$ 0.039 &  0.803$\pm$ 0.038     \\ 
5007\ [O\ {\sc iii}]\            &  1.634$\pm$ 0.036 &  1.446$\pm$ 0.036  &  1.363$\pm$ 0.080 &  1.202$\pm$ 0.079 &  2.436$\pm$ 0.114 &  2.358$\pm$ 0.112     \\ 
6300\ [O\ {\sc i}]\              &        ...        &        ...         &        ...        &        ...        &  0.017$\pm$ 0.008 &  0.013$\pm$ 0.006     \\ 
6312\ [S\ {\sc iii}]\            &        ...        &        ...         &        ...        &        ...        &  0.002$\pm$ 0.005 &  0.001$\pm$ 0.004     \\ 
6548\ [N\ {\sc ii}]\             &        ...        &        ...         &  0.040$\pm$ 0.070 &  0.033$\pm$ 0.065 &  0.032$\pm$ 0.005 &  0.024$\pm$ 0.004     \\ 
6563\ H$\alpha$\                 &  3.028$\pm$ 0.081 &  2.728$\pm$ 0.089  &  3.277$\pm$ 0.197 &  2.761$\pm$ 0.203 &  3.817$\pm$ 0.148 &  2.788$\pm$ 0.118     \\ 
6584\ [N\ {\sc ii}]\             &        ...        &        ...         &  0.140$\pm$ 0.087 &  0.116$\pm$ 0.081 &  0.101$\pm$ 0.014 &  0.073$\pm$ 0.010     \\ 
6678\ He\ {\sc i}\               &        ...        &        ...         &        ...        &        ...        &  0.025$\pm$ 0.002 &  0.018$\pm$ 0.002     \\ 
%                                       
   &  &  &  &  &  &  \\                        
C(H$\beta$)\ dex                   & \MC {2}{c}{0.01$\pm$0.04}      & \MC {2}{c}{0.10$\pm$0.08}             & \MC {2}{c}{0.41$\pm$0.05}                 \\
EW(abs)\ \AA\                      & \MC {2}{c}{4.60$\pm$0.20}      & \MC {2}{c}{1.75$\pm$0.19}             & \MC {2}{c}{0.05$\pm$0.32}                 \\
EW(H$\beta$)\ \AA\                 & \MC {2}{c}{35.5$\pm$0.6}       & \MC {2}{c}{13.9$\pm$0.6}              & \MC {2}{c}{65.5$\pm$2.4}                  \\  
\hline                                                                                                                                                   
$T_{\rm e}$(OIII)(K)\              & \MC {2}{c}{20538$\pm$2059}     & \MC {2}{c}{17833$\pm$2274}            & \MC {2}{c}{16103$\pm$657 }                \\
$T_{\rm e}$(OII)(K)\               & \MC {2}{c}{14847$\pm$345 }     & \MC {2}{c}{14855$\pm$369 }            & \MC {2}{c}{14391$\pm$245 }                \\
O$^{+}$/H$^{+}$($\times$10$^5$)\   & \MC {2}{c}{1.388$\pm$0.107}    & \MC {2}{c}{2.752$\pm$0.275}           & \MC {2}{c}{2.351$\pm$0.161}               \\ 
O$^{++}$/H$^{+}$($\times$10$^5$)\  & \MC {2}{c}{0.803$\pm$0.163}    & \MC {2}{c}{0.866$\pm$0.250}           & \MC {2}{c}{2.190$\pm$0.229}               \\ 
O/H($\times$10$^5$)\               & \MC {2}{c}{2.192$\pm$0.195}    & \MC {2}{c}{3.619$\pm$0.372}           & \MC {2}{c}{4.541$\pm$0.280}               \\ 
12+log(O/H)(d)\                    & \MC {2}{c}{7.34$\pm$0.04}      & \MC {2}{c}{...}                       & \MC {2}{c}{7.66$\pm$0.03}                 \\
12+log(O/H)(s)\                    & \MC {2}{c}{7.29$\pm$0.04}      & \MC {2}{c}{7.42$\pm$0.05}             & \MC {2}{c}{...}                              \\
12+log(O/H)(mse,c)\                & \MC {2}{c}{7.41$\pm$0.11}      & \MC {2}{c}{7.57$\pm$0.11}             & \MC {2}{c}{7.77$\pm$0.11}                 \\
12+log(O/H)(PT05)\                 & \MC {2}{c}{7.52$\pm$0.10}      & \MC {2}{c}{...}                       & \MC {2}{c}{7.81$\pm$0.10}                 \\
\MC{3}{l}{~~} \                                                                                                         
\end{tabular}                                                                                                           
 }
\end{table*}


==> addtab_wrong.tex <==
%PGC2807150.tex
%AGC208329a.tex
\begin{table*}
\centering{
\caption{Line intensities and derived parameters of PGC2807150 and AGC231980 from Table~4} %\ref{tab:wrong}}
\label{t:Intens1}
\begin{tabular}{lcccc} \hline
\rule{0pt}{10pt}
& \MC{2}{c}{PGC2807150=J1354+0414}    % \\ \hline
& \MC{2}{c}{AGC208329=J1015+0335}       \\ \hline
\rule{0pt}{10pt}
$\lambda_{0}$(\AA) Ion    & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$) & F($\lambda$)/F(H$\beta$)&I($\lambda$)/I(H$\beta$)  \\ \hline
%
3727\ [O\ {\sc ii}]\                  &  2.184$\pm$ 0.246 &  2.086$\pm$ 0.263  &  1.684$\pm$ 0.035 &  1.588$\pm$ 0.037         \\ 
3868\ [Ne\ {\sc iii}]\                &        ...        &        ...         &  0.303$\pm$ 0.013 &  0.286$\pm$ 0.013         \\ 
3889\ He\ {\sc i}\ +\ H8\             &        ...        &        ...         &  0.126$\pm$ 0.009 &  0.188$\pm$ 0.017         \\ 
3967\ [Ne\ {\sc iii}]\ +\ H7\         &        ...        &        ...         &  0.211$\pm$ 0.009 &  0.267$\pm$ 0.015         \\ 
4101\ H$\delta$\                      &  0.264$\pm$ 0.061 &  0.290$\pm$ 0.075  &  0.198$\pm$ 0.009 &  0.256$\pm$ 0.016         \\
4340\ H$\gamma$\                      &  0.437$\pm$ 0.067 &  0.454$\pm$ 0.077  &  0.403$\pm$ 0.021 &  0.440$\pm$ 0.026         \\
4363\ [O\ {\sc iii}]\                 &        ...        &        ...         &  0.036$\pm$ 0.017 &  0.034$\pm$ 0.017         \\ 
4861\ H$\beta$\                       &  1.000$\pm$ 0.114 &  1.000$\pm$ 0.131  &  1.000$\pm$ 0.021 &  1.000$\pm$ 0.023         \\ 
4959\ [O\ {\sc iii}]\                 &  0.494$\pm$ 0.061 &  0.472$\pm$ 0.061  &  1.420$\pm$ 0.027 &  1.339$\pm$ 0.027         \\ 
5007\ [O\ {\sc iii}]\                 &  1.081$\pm$ 0.111 &  1.032$\pm$ 0.111  &  4.254$\pm$ 0.070 &  4.012$\pm$ 0.070         \\ 
6548\ [N\ {\sc ii}]\                  &  0.023$\pm$ 0.103 &  0.022$\pm$ 0.103  &  0.039$\pm$ 0.012 &  0.036$\pm$ 0.012         \\ 
6563\ H$\alpha$\                      &  2.885$\pm$ 0.303 &  2.789$\pm$ 0.336  &  2.988$\pm$ 0.062 &  2.858$\pm$ 0.069         \\ 
6584\ [N\ {\sc ii}]\                  &  0.103$\pm$ 0.127 &  0.099$\pm$ 0.127  &  0.118$\pm$ 0.017 &  0.112$\pm$ 0.017         \\ 
%                                                                              
   &  &  &  &  \\                                                           
C(H$\beta$)\ dex                      & \MC {2}{c}{0.00$\pm$0.14}              & \MC {2}{c}{0.00$\pm$0.03}                     \\  
EW(abs)\ \AA\                         & \MC {2}{c}{0.60$\pm$0.70}              & \MC {2}{c}{5.80$\pm$0.65}                     \\   
EW(H$\beta$)\ \AA\                    & \MC {2}{c}{12.7$\pm$1.0}               & \MC {2}{c}{95.9$\pm$1.4}                      \\
\hline                                                                                                                
$T_{\rm e}$(OIII)(K)\                 & \MC {2}{c}{15412$\pm$1240}             & \MC {2}{c}{10991$\pm$1778}                    \\
$T_{\rm e}$(OII)(K)\                  & \MC {2}{c}{14104$\pm$568 }             & \MC {2}{c}{10888$\pm$1773}                    \\
O$^{+}$/H$^{+}$($\times$10$^5$)\      & \MC {2}{c}{2.298$\pm$0.418}            & \MC {2}{c}{4.467$\pm$2.933}                   \\ 
O$^{++}$/H$^{+}$($\times$10$^5$)\     & \MC {2}{c}{1.159$\pm$0.250}            & \MC {2}{c}{10.680$\pm$5.544}                  \\ 
O/H($\times$10$^5$)\                  & \MC {2}{c}{3.457$\pm$0.487}            & \MC {2}{c}{15.150$\pm$6.272}                  \\ 
12+log(O/H)(d)\                       & \MC {2}{c}{...          }              & \MC {2}{c}{8.18$\pm$0.18}                     \\
%12+log(O/H)(s)\                       & \MC {2}{c}{}                           & \MC {2}{c}{ }                                 \\
12+log(O/H)(mse,c)\                   & \MC {2}{c}{7.56$\pm$0.11}              & \MC {2}{c}{7.81$\pm$0.11}                     \\
12+log(O/H)(PT05)\                    & \MC {2}{c}{...}                        & \MC {2}{c}{7.85$\pm$0.10}                     \\
\MC{2}{l}{~~} \
\end{tabular}
 }
\end{table*}












